Model-Based Reparameterization Policy Gradient Methods: Theory and Practical Algorithms

ReParameterization (RP) Policy Gradient Methods (PGMs) have been widely adopted for continuous control tasks in robotics and computer graphics. However, recent studies have revealed that, when applied to long-term reinforcement learning problems, model-based RP PGMs may experience chaotic and non-smooth optimization landscapes with exploding gradient variance, which leads to slow convergence. This is in contrast to the conventional belief that reparameterization methods have low gradient estimation variance in problems such as training deep generative models. To comprehend this phenomenon, we conduct a theoretical examination of model-based RP PGMs and search for solutions to the optimization difficulties. Specifically, we analyze the convergence of the model-based RP PGMs and pinpoint the smoothness of function approximators as a major factor that affects the quality of gradient estimation. Based on our analysis, we propose a spectral normalization method to mitigate the exploding variance issue caused by long model unrolls. Our experimental results demonstrate that proper normalization significantly reduces the gradient variance of model-based RP PGMs. As a result, the performance of the proposed method is comparable or superior to other gradient estimators, such as the Likelihood Ratio (LR) gradient estimator. Our code is available at https://github.com/agentification/RP_PGM.

==> temp.tex <==
\section{Background}\label{sec_bg}
\noindent{\bf Reinforcement Learning.}
% \label{bg_rl}
We consider learning to optimize an infinite-horizon $\gamma$-discounted Markov Decision Process (MDP) over repeated episodes of interaction. We denote by $\mathcal{S}\subseteq\mathbb{R}^{d_s}$ and $\mathcal{A}\subseteq\mathbb{R}^{d_a}$ the state space and the action space, respectively. When taking an action $a\in\mathcal{A}$ at a state $s\in\mathcal{S}$, the agent receives a reward $r(s,a)$ and the MDP transits to a new state $s'$ according to probability $s'\sim f(\cdot\,|\, s,a)$.

%Define the stationary state-action distribution of policy $\pi$ as $\mu_\pi$. If the MDP is initialized at the stationary distribution $\mu_\pi$, then the state-action visitation measure $\sigma_\pi$ is the same as $\mu_\pi$.

We aim to find a policy $\pi$ that maps a state to an action distribution to maximize the expected cumulative reward. We denote by $V^\pi: \mathcal{S}\rightarrow \mathbb{R}$ and $Q^\pi: \mathcal{S}\times\mathcal{A}\rightarrow \mathbb{R}$ the state value function and the state-action value function associated with $\pi$, respectively, which are defined as follows,
\$
%V^\pi(s) = (1 - \gamma)\cdot\EE_{\pi, f}\biggl[\sum_{i=0}^\infty \gamma^i\cdot r(s_i, a_i)\,\bigg|\, s_0 = s\biggr],
Q^\pi(s, a) = (1 - \gamma)\cdot\EE_{\pi, f}\biggl[\sum_{i=0}^\infty \gamma^i\cdot r(s_i, a_i)\,\bigg|\, s_0 = s, a_0=a\biggr], \quad V^\pi(s) = \EE_{a\sim\pi}\biggl[Q^\pi(s, a)\biggr].
\$
Here $s\in\mathcal{S}$, $a\in\mathcal{A}$, and the expectation $\EE_{\pi, f}[\,\cdot\,]$ is taken with respect to the dynamic induced by the policy $\pi$ and the transition probability $f$.

We denote by $\zeta$ the initial state distribution. Under policy $\pi$, the state and state-action visitation measure $\nu_\pi(s)$ over $\mathcal{S}$ and $\sigma_\pi(s, a)$ over $\mathcal{S}\times\mathcal{A}$ are defined as follows,
\$
\nu_\pi(s) = (1 - \gamma) \cdot\sum_{i=0}^\infty\gamma^i \cdot\mathbb{P}(s_i = s),\qquad
\sigma_\pi(s, a) =  (1 - \gamma)\cdot \sum_{i=0}^\infty\gamma^i \cdot\mathbb{P}(s_i = s, a_i = a),
\$
where the summations are taken with respect to the trajectory induced by $s_0\sim \zeta$, $a_i\sim\pi(\cdot\,|\,s_i)$, and $s_{i+1}\sim f(\cdot\,|\,s_i, a_i)$. The objective $J(\pi)$ of RL is defined as the expected policy value as follows,
\#\label{rl_obj}
J(\pi) = \mathbb{E}_{s_0\sim\zeta}\bigl[V^{\pi}(s_0)\bigr] = \EE_{(s, a)\sim\sigma_\pi}\bigl[r(s, a)\bigr].
\#


%\vskip4pt
\noindent{\bf Stochastic Gradient Estimation.} The underlying problem of policy gradient, i.e., computing the gradient of an expectation with respect to the parameters of the sampling distribution, takes the form $\nabla_\theta\EE_{p(x;\theta)}[y(x)]$. To restore the RL objective, we can set $p(x;\theta)$ as the trajectory distribution conditioned on the policy parameter $\theta$ and $y(x)$ as the cumulative reward. In the sequel, we introduce two commonly used gradient estimators.%, which are LR (zeroth-order) and RP (first-order) gradient.

Likelihood Ratio (LR) Gradient (Zeroth-Order): By leveraging the \textit{score function}, LR gradients only require samples of the function values. Since $\nabla_\theta\log p(x;\theta) =\nabla_\theta p(x;\theta)/p(x;\theta)$, the LR gradient takes the form of
\#\label{lr_form}
\nabla_\theta\EE_{p(x;\theta)}\bigl[y(x)\bigr] = \EE_{p(x;\theta)}\bigl[y(x)\nabla_\theta\log p(x;\theta)\bigr].
\#

ReParameterization (RP) Gradient (First-Order): RP gradient benefits from the structural characteristics of the objective, i.e., how the overall objective is affected by the operations applied to the sources of randomness as they pass through the measure and into the cost function \citep{mohamed2020monte}. From the simulation property of continuous distribution, we have the following equivalence between direct and indirect ways of drawing samples,
\#\label{simu_cont}
\hat{x}\sim p(x;\theta)  \iff  \hat{x} = g(\epsilon; \theta),\, \epsilon\sim p.
\#
Derived from the \textit{law of the unconscious statistician} (LOTUS) \citep{grimmett2020probability}, i.e., $\EE_{p(x;\theta)}[y(x)] = \EE_{p(\epsilon)}[y(g(\epsilon; \theta))]$, the RP gradient can be formulated as
\$
\nabla_\theta\EE_{p(x;\theta)}\bigl[y(x)\bigr] = \EE_{p(\epsilon)}\Bigl[\nabla_\theta y\bigl(g(\epsilon; \theta)\bigr)\Bigr].
\$

%Based on this zeroth-order estimator, several policy gradient algorithms are proposed, e.g., REINFORCE \citep{williams1992simple} that is defined with a stochastic policy $\pi(a|s): \mathcal{S}\times\mathcal{A}\rightarrow \mathbb{R}$.
%Recent works have shown the global convergence of LR policy gradients \citep{bhandari2019global,agarwal2021theory,wang2019neural} under certain conditions. 
%$d^{\pi_\theta}(s)$ is the state visitation measure induced by $\pi_\theta$ over $\mathcal{S}$, defined as $d^{\pi_\theta}(s) = \sum_{t=0}^{H-1}\mathbb{P}(s_t=s)$ where $s_0\sim\zeta(\cdot), a_t\sim\pi(\cdot|s_t), s_{t+1} \sim \mathcal{P}(\cdot| s_h,a_h)$


%In RL, there are several algorithms that are built upon RP gradient (or pathwise gradient, policy-value gradient), including Deep Deterministic Policy Gradient (DDPG)\citep{lillicrap2015continuous}, Back-Propagation Through Time (BPTT) \citep{kurutach2018model,xu2022accelerated}, Stochastic Value Gradient (SVG) \citep{heess2015learning}, and Model-Augmented Actor-Critic (MAAC) \citep{clavera2020model}. It is experimentally observed recently \citep{parmas2018pipps,metz2021gradients} that RP gradients can suffer from large variance and the curse of chaos, the sensitive dependence on initial conditions due to the long chains of nonlinear mappings. In this work, we focus on the theoretical side studying how the gradient variance influences convergence and the principles to construct efficient RP policy-value gradient algorithms.


\section{Analytic Reparameterization Gradient in Reinforcement Learning}
\label{sec_rpg}
In this section, we present two fundamental \textit{analytic} forms of the RP gradient in RL. We first consider the Policy-Value Gradient (PVG) method, which is model-free and can be expanded sequentially to obtain the Analytic Policy Gradient (APG) method. Then we discuss potential obstacles that may arise when developing practical algorithms.

We consider a policy $\pi_\theta(s, \varsigma)$ with noise $\varsigma$ in continuous action spaces. To ensure that the first-order gradient through the value function is well-defined, we make the following continuity assumption.
\begin{assumption}[Continuous MDP]
\label{continuous}
We assume that $f(s'\,|\,s, a)$, $\pi_\theta(s,\varsigma)$, $r(s, a)$, and $\nabla_a r(s, a)$ are continuous in all parameters and variables $s$, $a$, $s'$.
\end{assumption}
\noindent{\bf Policy-Value Gradient.}
\label{mf_rp}
The reparameterization PVG takes the following general form,
\#\label{eq::general_rp}
\nabla_\theta J(\pi_\theta) =\EE_{s\sim\zeta, \varsigma\sim p}\Bigl[\nabla_\theta Q^{\pi_\theta}\bigl(s, \pi_\theta(s, \varsigma)\bigr)\Bigr].
\#

By performing sequential decision-making, any immediate action could lead to changes in all future states and rewards. Therefore, the value gradient $\nabla_\theta Q^{\pi_\theta}$ possesses a recursive structure. Adapted from the deterministic policy gradient theorem \citep{silver2014deterministic,lillicrap2015continuous} by taking stochasticity into consideration, we rewrite \eqref{eq::general_rp} as
\begin{flalign}
\text{PVG:} \hspace{-3.7cm}&&\nabla_\theta J(\pi_{\theta}) &= \EE_{s\sim\nu_\pi, \varsigma}\Bigl[\nabla_\theta\pi_\theta(s, \varsigma)\cdot\nabla_a Q^{\pi_\theta}(s, a)\big|_{a = \pi_\theta(s, \varsigma)}\Bigr].\notag
\end{flalign}
Here, $\nabla_a Q^{\pi_\theta}$ can be estimated using a critic, which leads to model-free frameworks \citep{heess2015learning,amos2021model}. Notably, as a result of the recursive structure of $\nabla_\theta Q^{\pi_\theta}$, the expectation is taken over the state visitation $\nu_\pi$ instead of the initial distribution $\zeta$.

By sequentially expanding PVG, we obtain the analytic representation of the policy gradient.
%the policy-value gradient can also be expanded in a dynamic way.
%through transition paths, which we turn our attention to in the following sections.

\noindent{\bf Analytic Policy Gradient.} Due to the simulation property of continuous distributions in \eqref{simu_cont}, we interchangeably write $a\sim\pi_\theta(\cdot\,|\,s)$ with $a=\pi_\theta(s, \varsigma)$ and $s'\sim f(\cdot\,|\,s, a)$ with $s'=f(s, a, \xi^*)$, where $\xi^*$ is sampled from the unknown distribution $p$. From the Bellman equation $V^{\pi_\theta}(s) = \EE_{\varsigma}[(1 - \gamma)\cdot r(s, \pi_\theta(s, \varsigma)) + \gamma\cdot\EE_{\xi^*}[V^{\pi_\theta}(f(s,  \pi_\theta(s, \varsigma), \xi^*))]]$, we obtain the following backward recursions of gradient,
\#\label{value_grad}
\nabla_\theta V^{\pi_\theta}(s) &= \EE_{\varsigma}\Bigl[(1 - \gamma)\nabla_a r \nabla_\theta\pi_\theta+ \gamma\EE_{\xi^*}\bigl[\nabla_{s'} V^{\pi_\theta}(s') \nabla_a f\nabla_\theta\pi_\theta + \nabla_\theta V^{\pi_\theta}(s')\bigr]\Bigr],\\
\label{value_grad_2}\nabla_s V^{\pi_\theta}(s) &= \EE_{\varsigma}\Bigl[(1 - \gamma)(\nabla_s r + \nabla_a r\nabla_s\pi_\theta) + \gamma\EE_{\xi^*}\bigl[\nabla_{s'} V^{\pi_\theta}(s')(\nabla_s f + \nabla_a f\nabla_s\pi_\theta)\bigr]\Bigr].
\#
See \S\ref{apg_approx} for detailed derivations of \eqref{value_grad} and \eqref{value_grad_2}. Now we have the RP gradient backpropagated through the transition path starting at $s$. By taking an expectation over the initial state distribution, we obtain the Analytic Policy Gradient (APG) that takes the following form,
\begin{flalign}
\text{APG:} \hspace{-5.4cm}&&\nabla_\theta J(\pi_{\theta}) = \EE_{s\sim\zeta}\bigl[\nabla_\theta V^{\pi_\theta}(s)\bigr].\notag
\end{flalign}
There remain challenges when developing practical algorithms: (1) the above formulas require the gradient information of the transition function $f$. In this work, however, we consider a common RL setting where $f$ is unknown and needs to be fitted by a model. It is thus natural to ask how the properties of the model (e.g., prediction accuracy and model smoothness) affect the gradient estimation and the convergence of the resulting algorithms, and (2) even if we have access to an accurate model, unrolling it over full sequences faces practical difficulties. The memory and computational cost scale linearly with the unroll length. Long chains of nonlinear mappings can also lead to exploding or vanishing gradients and even worse, chaotic phenomenons \citep{bollt2000controlling} and difficulty in optimization \citep{pascanu2013difficulty,maclaurin2015gradient,vicol2021unbiased,metz2019understanding}. These difficulties demand some form of truncation when performing RP PGMs.

\section{Model-Based RP Policy Gradient Methods}
\label{sec_mb_rp_pgm}
%In this section, we present the model-based RP PG frameworks built on model value expansion.
%In this section, we introduce Model Value Expansion (MVE) for model truncation and present two model-based RP policy gradient frameworks built upon MVE.
Through the application of Model Value Expansion (MVE) for model truncation, this section unveils two RP policy gradient frameworks constructed upon MVE.
\subsection{$h$-Step Model Value Expansion}
To handle the difficulties inherent in full unrolls, many algorithms employ direct truncation, where the long sequence is broken down into short sub-sequences and backpropagation is applied accordingly, e.g., Truncated BPTT \cite{werbos1990backpropagation}. However, such an approach over-prioritizes short-term dependencies, which leads to biased gradient estimates.

In model-based RL (MBRL), one viable solution is to adopt the $h$-step Model Value Expansion \cite{feinberg2018model}, which decomposes the value estimation $\hat{V}^\pi(s)$ into the rewards gleaned from the learned model and a residual estimated by a critic function $\hat{Q}_\omega$, that is,
\$
\hat{V}^{\pi_\theta}(s) = (1 - \gamma)\cdot\Biggl(\sum_{i=0}^{h-1} \gamma^i\cdot r(\hat{s}_i, \hat{a}_i) + \gamma^h\cdot\hat{Q}_\omega(\hat{s}_{h}, \hat{a}_{h})\Biggr),
\$
where $\hat{s}_{0} = s$, $\hat{a}_{i}=\pi_\theta(\hat{s}_{i}, \varsigma)$, and $\hat{s}_{i+1}=\hat{f}_\psi(\hat{s}_i, \hat{a}_i, \xi)$. Here, the noise variables $\varsigma$ and $\xi$ can be sampled from the fixed distributions or inferred from the real samples, which we will discuss in the following section.

\subsection{Model-Based RP Gradient Estimation}
\label{sec::model_use}
%With function approximated model $\hat{f}$ and critic $\hat{Q}_\omega$, the simulated trajectory under a stochastic policy $\pi: \mathcal{S}\rightarrow\mathcal{A}$ can be used for value estimation, by sampling and replacing $f$, $Q^\pi$ with $\hat{f}$, $\hat{Q}_\omega$, respectively.
%By taking the pathwise gradient with respect to the policy parameter $\theta$ in the MVE formula \eqref{hmve}, we obtain the following frameworks with the difference lies in whether the samples used for gradient estimation come from model unrolls or from real trajectories.
Utilizing the pathwise gradient with respect to $\theta$, we present the following two frameworks.

%\vskip4pt
\noindent{\bf Model Derivatives on Predictions (DP).} A straightforward way to compute the first-order gradient is to link the reward, model, policy, and critic together and backpropagate through them. Specifically, the differentiation is carried out on the trajectories simulated by the model $\hat{f}_\psi$, which serves as a tool for \textit{both} the prediction of states and the evaluation of derivatives. The corresponding RP-DP estimator of gradient $\nabla_\theta J(\pi_{\theta})$ is denoted as $\hat{\nabla}_\theta^\text{DP} J(\pi_{\theta})$, which takes the form of
\#\label{DP_ge}
\hat{\nabla}_\theta^\text{DP} J(\pi_{\theta}) &= \frac{1}{N}\sum_{n=1}^N \nabla_\theta\biggl(\sum_{i=0}^{h-1} \gamma^i\cdot r(\hat{s}_{i,n}, \hat{a}_{i,n}) + \gamma^h\cdot \hat{Q}_\omega(\hat{s}_{h,n}, \hat{a}_{h,n})\biggr),
\#
where $\hat{s}_{0,n}\sim\mu_{\pi_\theta}$, $\hat{a}_{i,n}=\pi_\theta(\hat{s}_{i,n}, \varsigma_n)$, and $\hat{s}_{i+1, n}=\hat{f}_\psi(\hat{s}_{i,n}, \hat{a}_{i, n}, \xi_n)$ with noises $\varsigma_n\sim p(\varsigma)$ and $\xi_n\sim p(\xi)$. Here, $\mu_{\pi_\theta}$ is the distribution where the initial states of the simulated trajectories are sampled. In Section \ref{sec_main_result}, we study a general form of $\mu_{\pi_\theta}$ that is a mixture of the initial state distribution $\zeta$ and the state visitation $\nu_{\pi_\theta}$.

Various algorithms can be instantiated from \eqref{DP_ge} with different choices of $h$. When $h=0$, the framework reduces to model-free policy gradients, such as RP($0$) \citep{amos2021model} and the variants of DDPG \citep{lillicrap2015continuous}, e.g., SAC \citep{haarnoja2018soft}. When $h\rightarrow\infty$, the resulting algorithm is BPTT \citep{grzeszczuk1998neuroanimator,degrave2019differentiable,bastani2020sample} where only the model is learned. Recent model-based approaches, such as MAAC \citep{clavera2020model} and related algorithms \citep{parmas2018pipps,amos2021model,li2021gradient}, require a carefully selected $h$.

%\vskip4pt
\noindent{\bf Model Derivatives on Real Samples (DR).} An alternative approach is to use the learned differentiable model solely for the calculation of derivatives, with the aid of Monte-Carlo estimates obtained from \textit{real} samples. By replacing $\nabla_a f, \nabla_s f$ in \eqref{value_grad}-\eqref{value_grad_2} with $\nabla_a\hat{f}_\psi, \nabla_a\hat{f}_\psi$ and setting the termination of backpropagation at the $h$-th step as $\hat{\nabla} V^{\pi_\theta}(\hat{s}_{h, n}) = \nabla\hat{V}_\omega(\hat{s}_{h, n})$, we are able to derive a dynamic representation of $\hat{\nabla}_\theta V^{\pi_\theta}$, which we defer to \S\ref{apg_approx}. 

The corresponding RP-DR gradient estimator takes the following form,
\#\label{DR_ge}
\hspace{-0.1cm}\hat{\nabla}_\theta^\text{DR} J(\pi_{\theta}) = \frac{1}{N}\sum_{n=1}^N \hat{\nabla}_\theta V^{\pi_\theta}(\hat{s}_{0,n}),
%= \frac{1}{N}\sum_{n=1}^N \nabla_\theta\biggl(\sum_{i=0}^{h-1} \gamma^i r(\hat{s}_{i,n}, \hat{a}_{i,n}) +\gamma^h \hat{Q}_\omega(\hat{s}_{h,n}, \hat{a}_{h,n})\biggr),
\#
where $\hat{s}_{0,n}\sim\mu_{\pi_\theta}$. Equation \eqref{DR_ge} can be specified as \eqref{app_eq_dr}, which is in the same format as \eqref{DP_ge}, but with the noise variables $\varsigma_n$, $\xi_n$ inferred from the real data sample $(s_{i}, a_{i}, s_{i+1})$ via the relation $a_{i} = \pi_\theta(s_{i}, \varsigma_n)$ and $s_{i+1} = \hat{f}_\psi(s_{i}, a_{i}, \xi_n)$ (see \S\ref{apg_approx} for details). Algorithms such as SVG \citep{heess2015learning} and its variants \citep{abbeel2006using,atkeson2012efficient} are examples of this method.

%In this framework, the model accuracy will only affect one-step derivative error, avoiding compounding error when the state's transit. As a trade-off of lower bias, the gradient variance might be high since it depends on the property of the $true$ underlying dynamics instead of the estimated model where regularity can be imposed (e.g., Lipschitz continuity).

\subsection{Algorithmic Framework}
\begin{wrapfigure}{R}{0.56\textwidth}
\begin{minipage}{0.56\textwidth}
\vspace{-0.40cm}
\begin{algorithm}[H]
\caption{Model-Based RP Policy Gradient Method}
\begin{algorithmic}[1]\label{alg::RP}
\REQUIRE Number of iterations $T$, learning rate $\eta$, batch size $N$, state distribution $\mu(\cdot)$
%\STATE Initialize replay buffer $\mathcal{D} = \emptyset$
\FOR{iteration $t \in [T]$}
%\STATE Sample $\mathcal{B}=\{\{(s_{i,n}, a_{i,n})\}_{i\in[h]}\}_{n\in[N]}$ from $\mathcal{D}$
\STATE \label{line::model}
Update the model parameter $\psi_{t}$ by MSE or MLE
\STATE \label{line::policy_eval}
Update the critic parameter $\omega_{t}$ by performing TD
\STATE Sample states from $\mu_{\pi_t}$ and estimate $\hat\nabla_\theta J(\pi_{\theta_t})=\hat{\nabla}_\theta^\text{DP} J(\pi_{\theta_t})$ \eqref{DP_ge} or $\hat{\nabla}_\theta^\text{DR} J(\pi_{\theta_t})$ \eqref{DR_ge}
\STATE{Update the policy parameter $\theta_{t}$ by $
\theta_{t+1} \leftarrow\theta_t + \eta\cdot\hat{\nabla}_\theta J(\pi_{\theta_t})$ and execute $\pi_{\theta_{t+1}}$
}
\ENDFOR 
\STATE {\bf Output:} $\{ \pi_{\theta_t}\}_{t\in[T]}$
\end{algorithmic}
\end{algorithm}
  \vspace{-10pt}
\end{minipage}
\end{wrapfigure}
%\vskip3pt
The pseudocode of model-based RP PGMs is presented in Algorithm \ref{alg::RP}, where three update procedures are performed iteratively. In other words, the policy, model, and critic are updated at each iteration $t\in[T]$, generating sequences of $\{\pi_{\theta_t}\}_{t\in[T+1]}$, $\{\hat{f}_{\psi_t}\}_{t\in[T]}$, and $\{\hat{Q}_{\omega_t}\}_{t\in[T]}$, respectively.


\noindent{\bf Policy Update.} The update rule for the policy parameter $\theta$ with learning rate $\eta$ is as follows,
\#\label{eq_policy_upd}
\theta_{t+1} \leftarrow \theta_t + \eta\cdot\hat{\nabla}_\theta J(\pi_{\theta_t}),
\#
where $\hat{\nabla}_\theta J(\pi_{\theta_t})$ can be specified as $\hat{\nabla}_\theta^\text{DP} J(\pi_{\theta_t})$ or $\hat{\nabla}_\theta^\text{DR} J(\pi_{\theta_t})$.
%by the two gradient estimators discussed earlier: when the model is used for derivatives calculation and state prediction, i.e., $\hat{\nabla}_\theta^\text{DP} J(\pi_{\theta})$ defined in \eqref{DP_ge}; or when the model derivatives are calculated on real samples, i.e., $\hat{\nabla}_\theta^\text{DR} J(\pi_{\theta})$ defined in \eqref{DR_ge}.
%At iteration $t$, let the policy parameter space be $\mathcal{B}(R) = \{\theta_t: \|\theta_t - \Tilde{\theta}\|_2 \leq R\}$, where $R$ is the radius of the $l_2$ ball centered at $\Tilde{\theta}$. Here, $\Tilde{\theta}$ can be set to $\theta_{t-1}$, the policy parameter at the last iteration, which restricts $\theta_t$ to be updated within a trust-region. Or $\Tilde{\theta}$ can be simply set to the initialization of $\theta$.

%Define a projection operator $\Pi_{\mathcal{B}}(\theta) = \argmin_{\theta'\in\mathcal{B}}\|\theta' - \theta\|_2$. 
%To approximate the (stochastic) environment dynamics, model-based RL learns a forward model that predicts how the system will evolve when applying action $a$ at state $s$. 
%A straightforward way for learning a state-predictive model is to learn a deterministic function as the mean of transition, by minimizing the mean squared error (MSE) between the predictions and ground truth. An alternative approach is to fit a probabilistic function by performing maximum likelihood estimation (MLE) on the sampled data.
%Hereafter, the stochastic model we study is a deterministic NN with additive noise, i.e., $\hat{s}_{i+1} = \hat{f}(s_i, a_i; \psi) + \xi$ \yan{is it $s_{i+1}$?}, where $\xi\sim p(\xi)$ is sampled from any tractable distribution.
%We study the probabilistic NN with the form of $\hat{s}_{i+1} \sim \hat{f}(\cdot|s_i, a_i; \psi)$. For instance, $\hat{f}$ can output a Gaussian distribution with diagonal covariances parameterized by $\psi$.

%Denote the transition prediction error $\epsilon_f$ at iteration $t$ as the maximum expected total variation distance between the true dynamics $f$ and the approximated $\hat{f}_{\psi_t}$, defined by
%\#\label{model_error}
%%\epsilon_f(t) := \max_{(s, a)\in\mathcal{S}\times\mathcal{A}} D_{\text{TV}}\bigl(f(\cdot\,|\,s, a), \hat{f}_{\psi_t}(\cdot\,|\,s, a)\bigr),
%\epsilon_f(t) := \max_{i\in[h]}\EE_{\mathbb{P}_i(s, a)}\Bigl[D_{\text{TV}}\bigl(f(\cdot\,|\,s_i, a_i), \hat{f}_{\psi_t}(\cdot\,|\,s_i, a_i)\bigr)\Bigr],
%%\epsilon_f(t): = \EE_{(s, a)\sim\sigma_{\pi_t}}\Bigl[D_{\text{TV}}\bigl(f(\cdot\,|\,s, a), \hat{f}_{\psi_t}(\cdot\,|\,s, a)\bigr)\Bigr],
%\#
%where $\mathbb{P}_i(s, a)$ is the true state-action distribution at timestep $i$, defined as $\mathbb{P}_i(s, a):= \mathbb{P}(s_i=s, a_i=a)$ with $s_0\sim \zeta(\cdot)$, $a_j\sim\pi_t(\cdot\,|\,s_j)$, and $s_{j+1}\sim f(\cdot\,|\,s_j, a_j)$.
%%Notably, $\epsilon_f$ regulates the transition prediction error at each state-action pair. Compared to the model error definition where the expectation is taken over the state-action visitation under $\pi_t$, the representation of $\epsilon_f$ requires an additional measure of the model complexity (e.g., Eluder Dimension \cite{osband2014model}), such that the generalizability of the model class is captured.
%\vskip3pt
\noindent{\bf Model Update.}
By predicting the mean of transition with minimized mean squared error (MSE) or fitting a probabilistic model with maximum likelihood estimation (MLE), canonical MBRL methods learn forward models that predict how the system evolves when an action $a$ is taken at state $s$. 

However, accurate state predictions do not imply accurate RP gradient estimation. Thus, we introduce $\epsilon_f(t)$ to represent the model (gradient) error at iteration $t$, defined as
\#\label{error_model_def}
\epsilon_f(t) = \max_{i\in[h]}\,\EE_{\mathbb{P}(s_i, a_i), \mathbb{P}(\hat{s}_i, \hat{a}_i)}\biggl[\biggl\|\frac{\partial s_i}{\partial s_{i-1}} - \frac{\partial\hat{s}_i}{\partial\hat{s}_{i-1}}\biggr\|_2 + \biggl\|\frac{\partial s_i}{\partial a_{i-1}} - \frac{\partial\hat{s}_i}{\partial\hat{a}_{i-1}}\biggr\|_2\biggr],
%\max_{i\in[h]}\,\EE_{\mathbb{P}(s_i, a_i), \mathbb{P}(\hat{s}_i, \hat{a}_i)}\Bigl[\big\|\nabla_s f(s, a, \xi^*) - \nabla_{\hat{s}} \hat{f}_t(\hat{s}, \hat{a}, \xi)\big\|_2\Bigr] \leq \epsilon_f(t),\notag\\
%\max_{i\in[h]}\,\EE_{\mathbb{P}(s_i, a_i), \mathbb{P}(\hat{s}_i, \hat{a}_i)}\Bigl[\big\|\nabla_a f(s, a, \xi^*) - \nabla_{\hat{a}} \hat{f}_t(\hat{s}, \hat{a}, \xi)\big\|_2\Bigr] \leq \epsilon_f(t),
%\epsilon_f(t) := \max_{i}\EE_{(s, a)\sim\mathbb{P}(s_i, a_i)}\Bigl[\big\|\nabla_s \hat{f}(s, a, \xi) - \nabla_s f(s, a, \xi^*)\big\|_2 + \big\|\nabla_a \hat{f}(s, a, \xi) - \nabla_a f(s, a, \xi^*)\big\|_2\Bigl].
\#
%where $s_0\sim \zeta(\cdot)$, $a_j\sim\pi_t(\cdot\,|\,s_j)$, and $s_{j+1}\sim f(\cdot\,|\,s_j, a_j)$. 
where $\mathbb{P}(s_i, a_i)$ is the true state-action distribution at the $i$-th timestep by following $s_0\sim \nu_{\pi_{\theta_t}}$, $a_j\sim\pi_{\theta_t}(\cdot\,|\,s_j)$, $s_{j+1}\sim f(\cdot\,|\,s_j, a_j)$, with policy and transition noise sampled from a fixed distribution. Similarly, $\mathbb{P}(\hat{s}_i, \hat{a}_i)$ is the model rollout distribution at the $i$-th timestep by following $\hat{s}_0\sim \nu_{\pi_{\theta_t}}$, $\hat{a}_j\sim\pi_{\theta_t}(\cdot\,|\,\hat{s}_j)$, $\hat{s}_{j+1}\sim \hat{f}_{\psi_t}(\cdot\,|\,\hat{s}_j, \hat{a}_j)$, where the noise is sampled when we use RP-DP gradient estimator and is inferred from real samples when we use RP-DR gradient estimator (in this case $\mathbb{P}(\hat{s}_i, \hat{a}_i) = \mathbb{P}(s_i, a_i)$).

In MBRL, it is common to learn a state-predictive model that can make multi-step predictions. However, this presents a challenge in reconciling the discrepancy between minimizing state prediction error and the gradient error of the model. Although it is natural to consider regularizing the models' directional derivatives to be consistent with the samples \citep{li2021gradient}, we contend that the use of state-predictive models does \textit{not} cripple our analysis of gradient bias based on $\epsilon_f$: For learned models that extrapolate beyond the visited regions, the gradient error can still be bounded via finite difference. In other words, $\epsilon_f$ can be expressed as the mean squared training error with an additional measure of the model class complexity to capture its generalizability.  This same argument can also be applied to the case of learning a critic through temporal difference.

%In model-based RL, it is common to learn a (multi-step) \textit{state}-predictive model, where the objective mismatch issue arises here between minimizing the state prediction error and the model gradient error in \eqref{error_model_def}. Although it is natural to consider explicitly regularizing the models' directional derivatives to be consistent with the samples \citep{li2021gradient}, we argue that the naive adoption of state-predictive models does \textit{not} cripple our analysis of gradient bias based on $\epsilon_f$: For learned models that extrapolate beyond the visited regions, the gradient error can still be bounded via finite difference. In other words, $\epsilon_f$ can be expressed as the mean squared training error with an additional measure of the model class complexity to capture its generalizability. A similar argument also holds for learning a critic by temporal difference.

%Since there is an objective mismatch issue between minimizing the state prediction error and the gradient error, it might be natural to consider learning the model whose directional derivative is consistent with the samples. However, we mainly consider the (multi-step) state-prediction model in our implementation due to its universality. However, we observe in experiments that multi-step state-predictive models suffice to give good results. This is because if the forward model learned in visited regions can extrapolate well, the gradient error can be bounded with finite difference approximation. In other words, $\epsilon_f$ might be expressed as MSE with an additional measure of the model complexity, with which the generalizability of the model class is captured. A similar argument also holds for learning a critic with temporal difference.

%\vskip3pt
\noindent{\bf Critic Update.}
For any policy $\pi$, its value function $Q^\pi$ satisfies the Bellman equation, which has a unique solution. In other words, $Q = \mathcal{T}^\pi Q$ if and only if $Q = Q^\pi$. The Bellman operator $\mathcal{T}^\pi$ is defined for any $(s, a)\in\mathcal{S}\times\mathcal{A}$ as
\$
\mathcal{T}^\pi Q(s, a) = \EE_{\pi, f}\bigl[(1 - \gamma)\cdot r(s, a) + \gamma\cdot Q(s', a')\bigr].
\$
%We aim to approximate the state-action value $Q$ with a critic $\hat{Q}_\omega$. Define the critic error $\epsilon_Q$ as
%\#\label{critic_error}
%%\epsilon_Q(t) :=\max_{(s, a)\in\mathcal{S}\times\mathcal{A}}\bigl|Q^{\pi_{\theta_t}}(s, a) - \hat{Q}_{\omega_t}(s, a)\bigr|.
%\epsilon_Q(t) :=\EE_{(s, a)\sim\sigma_{\pi_t}}\Bigl[\bigl|Q^{\pi_{\theta_t}}(s, a) - \hat{Q}_{\omega_t}(s, a)\bigr|\Bigr].
%\#
We aim to approximate the state-action value function $Q^\pi$ with a critic $\hat{Q}_\omega$. Due to the solution uniqueness of the Bellman equation, it can be achieved by minimizing the mean-squared Bellman error $\EE[(\hat{Q}_\omega(s, a) - \mathcal{T}^{\pi}\hat{Q}_\omega(s, a))^2]$ via Temporal Difference (TD) \citep{sutton1988learning,cai2019neural}. We define the critic error at the $t$-th iteration as follows,
\#\label{error_critic_def}
%\epsilon_v(t) := \EE_{(s, a)\sim\mathbb{P}(s_h, a_h)}\Bigl[\big\|\nabla_s \hat{V}(s) - \nabla_s V(s)\big\|_2\Bigl].
\epsilon_v(t) &= \alpha^2\cdot\EE_{\mathbb{P}(s_h, a_h), \mathbb{P}(\hat{s}_h, \hat{a}_h)}\biggl[\biggl\|\frac{\partial Q^{\pi_{\theta_t}}}{\partial s} - \frac{\partial\hat{Q}_{\omega_t}}{\partial\hat{s}}\biggr\|_2 + \biggl\|\frac{\partial Q^{\pi_{\theta_t}}}{\partial a} - \frac{\partial\hat{Q}_{\omega_t}}{\partial\hat{a}}\biggr\|_2\biggr],
\#
where $\alpha= (1 - \gamma) / \gamma^h$ and $\mathbb{P}(s_h, a_h)$, $\mathbb{P}(\hat{s}_h, \hat{a}_h)$ are distributions at timestep $h$ with the same definition as in \eqref{error_model_def}. The inclusion of $\alpha^2$ ensures that the critic error remains in alignment with the single-step model error $\epsilon_f$: (1) the critic estimates the tail terms that occur after $h$ steps in the model expansion, therefore the step-average critic error should be inversely proportional to the tail discount summation $\sum_{i=h}^\infty\gamma^i = 1 / \alpha$, and (2) the quadratic form shares similarities with the canonical MBRL analysis -- the cumulative error of the model trajectories scales linearly with the single-step prediction error and quadratically with the considered horizon (i.e., tail after the $h$-th step). This is because the cumulative error is linear in the considered horizon and the maximum state discrepancy, which is linear in the single-step error and, again, the horizon \citep{janner2019trust}. 


\section{Main Results}\label{sec_main_result}
%\vspace{-0.2cm}
In what follows, we present our main theoretical results, whose detailed proofs are deferred to \S\ref{app_proof}. Specifically, we analyze the convergence of model-based RP PGMs and, more importantly, study the correlation between the convergence rate, gradient bias, variance, smoothness of the model, and approximation error. Based on our theory, we propose various algorithmic designs for model-based RP PGMs.
%(Hereafter, we consider stochastic policy and dynamics with additive subgaussian noise, i.e., $\hat{a} = \pi_\theta(\hat{s}) + \varsigma$ and $\hat{s}' = \hat{f}(\hat{s}, \hat{a}) + \xi$. The noise distribution $p(\varsigma)$ and $p(\xi)$ are $\sigma_\eta$- and $\sigma_\xi$-subgaussian, respectively.)
%Denote $\hat{f}_\theta(s,\varsigma) = \hat{f}(s, \pi_\theta(s)+ \varsigma)$ and ${r}_\theta(s, \varsigma) = {r}(s, \pi_\theta(s) + \varsigma)$.

To begin with, we impose a common regularity condition on the policy functions following previous works \citep{xu2019sample,pirotta2015policy,zhang2020global,agarwal2021theory}. The assumption below essentially ensures the smoothness of the objective $J(\pi_\theta)$, which is required by most existing analyses of policy gradient methods \citep{wang2019neural,bastani2020sample,agarwal2020optimality}.
\begin{assumption}[Lipschitz and Bounded Score Function]
\label{assu_smooth_policy}
We assume that the score function of policy $\pi_\theta$ is Lipschitz continuous and has bounded norm $\forall (s, a)\in\mathcal{S}\times\mathcal{A}$, that is,
%for any $\theta\in\Theta$ in the policy parameter space $\Theta$,
\$
\big\|\log\pi_{\theta_1}(a\,|\,s) - \log\pi_{\theta_2}(a\,|\,s)\big\|_2\leq L_1\cdot\|\theta_1 - \theta_2\|_2,\quad
\big\|\log\pi_{\theta}(a\,|\,s)\big\|_2\leq B_\theta.
\$
\end{assumption}

We characterize the convergence of RP PGMs by first providing the following proposition.
%Since $\theta$ is restricted to stay in the $\mathcal{B}$ space, a stationary point $\hat{\theta}\in\mathcal{B}$ of $J(\pi_\theta)$ is defined as $\nabla_\theta J(\pi_{\hat{\theta}})^\top(\theta - \hat{\theta}) \leq 0$. For all $t\in[T]$, we define the gradient mapping at $\theta_t$ as

%Since $\hat{\theta}\in\mathcal{B}$ is a stationary point if and only if the gradient mapping at $\hat{\theta}$ is a zero vector, we character the convergence of the gradient mapping with the following proposition.

\begin{proposition}[Convergence to Stationary Point]
\label{prop1}
We define the gradient bias $b_t$ and variance $v_t$ as
\$
b_t = \big\| \nabla_{\theta}J(\pi_{\theta_t}) - \EE\bigl[\hat{\nabla}_{\theta} J(\pi_{\theta_t})\bigr] \big\|_2,\quad
v_t = \EE\bigl[\big\|\hat{\nabla}_{\theta} J(\pi_{\theta_t}) - \EE\bigl[\hat{\nabla}_{\theta} J(\pi_{\theta_t})\bigr]\big\|_2^2\bigr].
\$
Suppose the absolute value of the reward $r(s,a)$ is bounded by $|r(s,a)|\leq r_\text{m}$ for $(s, a)\in\mathcal{S}\times\mathcal{A}$. Let $\delta = \sup\|\theta\|_2$, $L = r_\text{m}\cdot L_1 / (1 - \gamma)^2 + (1 + \gamma)\cdot r_\text{m}\cdot B_\theta^2 / (1 - \gamma)^3$, and $c = (\eta - L\eta^2)^{-1}$. It then holds for $T \geq 4L^2$ that
\$
\min_{t\in[T]}\EE\Bigl[\big\|\nabla_{\theta}J(\pi_{\theta_t})\big\|_2^2\Bigr]\leq \frac{4c}{T}\cdot\EE\big[J(\pi_{\theta_T}) - J(\pi_{\theta_1})\big] + \frac{4}{T} \biggl(\sum_{t=0}^{T-1} c(2\delta\cdot b_{t} +  \frac{\eta}{2}\cdot v_{t}) + b_t^2 + v_t\biggr).
\$
%\vspace{-0.2cm}
%b_t =\Big\|\nabla_{\theta}J(\pi_{\theta_t}) - \EE\bigl[\hat{\nabla}_\theta J(\pi_{\theta_t})\bigl]\Big\|_2,\quad v_t = \EE\Bigl[\Big\|\hat{\nabla}_{\theta}J(\pi_{\theta_t}) - \EE\bigl[\hat{\nabla}_{\theta}J(\pi_{\theta_t})\bigr]\Big\|_2^2\Bigr].
\end{proposition}\vspace{-0.2cm}
Proposition \ref{prop1} illustrates the interdependence between the convergence and the variance, bias of the gradient estimators. In order for model-based RP PGMs to converge, it is imperative to maintain both the variance and bias at sublinear growth rates. Prior to examining the upper bound of $b_t$ and $v_t$, we make the following Lipschitz assumption, which has been implemented in a plethora of preceding studies \citep{pirotta2015policy,clavera2020model,li2021gradient}.

\begin{assumption}[Lipschitz Continuity]
\label{lip_assumption}
We assume that $r(s, a)$, $f(s, a, \xi^*)$, $\hat{f}_\psi(s, a, \xi)$, $\pi_\theta(s, \varsigma)$, $\hat{Q}_\omega(s, a)$ are $L_r, L_f, L_{\hat{f}}, L_\pi, L_{\hat{Q}}$ Lipschitz continuous (details in \S\ref{appendix_assump}).\vspace{-0.2cm}
\end{assumption}

Let $\Tilde{L}_{g} = \max\{L_g, 1\}$, where $L_g$ is the Lipschitz of function $g$. We have the following result for gradient variance.

\begin{proposition}[Gradient Variance]
\label{prop::grad_var}
Under Assumption \ref{lip_assumption}, for any $t\in[T]$, the gradient variance of the estimator $\hat{\nabla}_\theta J(\pi_{\theta})$, which can be specified as $\hat{\nabla}_\theta^\text{DP} J(\pi_{\theta})$ or $\hat{\nabla}_\theta^\text{DR} J(\pi_{\theta})$, can be bounded by
\$
v_t = O\biggl(h^4\biggl(\frac{1-\gamma^h}{1-\gamma}\biggr)^2 \Tilde{L}_{\hat{f}}^{4h}\Tilde{L}_\pi^{4h} / N + \gamma^{2h}h^4 \Tilde{L}_{\hat{f}}^{4h}\Tilde{L}_\pi^{4h} / N\biggr).
\$
%\vspace{-0.2cm}
\end{proposition}
We observe that the variance upper bound exhibits a polynomial dependence on the Lipschitz continuity of the model and policy, where the degrees are linear in the model unroll length. This makes sense intuitively, as the transition can be highly chaotic when $L_{\hat{f}}>1$ and $L_\pi>1$. This can result in diverging trajectories and variable gradient directions during training, leading to significant variance in the gradients.

%Therefore, when the underlying dynamic of the MDP is complex and contact-rich \citep{suh2022differentiable,xu2022accelerated}, model-based RP PGMs have their own advantages by leveraging smooth proxy models to significantly reduce the gradient variance. 

\begin{remark}
Model-based RP PGMs with non-smooth models and policies can suffer from large variance and highly non-smooth loss landscapes, which can lead to slow convergence or failure during training even in simple toy examples \citep{parmas2018pipps,metz2021gradients,suh2022differentiable}. Proposition \ref{prop::grad_var} suggests that one can add smoothness regularization to avoid exploding gradient variance. See our discussion at the end of this section for more details.\hspace{-0.5cm}
\end{remark}

%Model-based RP PGMs have their own advantages by leveraging proxy models for variance reduction. By enforcing the smoothness of the model, the gradient variance is reduced without burden when the underlying transition is smooth. However, for non-smooth dynamics (e.g., complex or contact-rich tasks \citep{suh2022differentiable,pang2022global}), this may introduce additional bias due to the increased model estimation error, which demands the trade-off between the model error and gradient variance. Interestingly, our empirical study shows that smoothness regularization improves performance even with the cost of a higher bias.
\textit{Model-based} RP PGMs possess unique advantages by utilizing proxy models for variance reduction. By enforcing the smoothness of the model, the gradient variance is reduced without a burden when the underlying transition is smooth. However, in cases of non-smooth dynamics, doing so may introduce additional bias due to increased model estimation error. This necessitates a trade-off between the model error and gradient variance. Nevertheless, our empirical study demonstrates that smoothness regularization improves performance in robotic locomotion tasks, despite the cost of increased bias.

%\begin{assumption}[Lipschitz Q-Value]
%\label{lip_q}
%Assume the state-action value is $L_Q$ Lipschitz continuous.
%\end{assumption}
%For this reason, we define the following state-action visitation measure over $\mathcal{S}$:
%\#\label{def::new_sigma}
%\overline{\sigma}_1(s, a) = \sum_{i=h}^\infty\gamma^{i - h} \cdot\mathbb{P}(s_i = s, a_i=a),\quad \overline{\sigma}_2(s, a) = \mathbb{P}(s_h = s, a_h = a),
%\#
%where $s_0\sim \zeta$, $a_i\sim\pi(\cdot\,|\,s_i)$, and $s_{i+1}\sim f(\cdot\,|\,s_i, a_i)$.


Next, we study the gradient bias. We consider the case where the state distribution $\mu_\pi$, which is used for estimating the RP gradient, is a mixture of the initial distribution $\zeta$ of the MDP and the state visitation $\nu_\pi$. In other words, we consider $\mu_\pi = \beta\cdot\nu_\pi + (1 - \beta)\cdot\zeta$, where $\beta\in[0, 1]$. This form is of particular interest as it encompasses various state sampling schemes that can be employed, such as when $h=0$ and $h\rightarrow\infty$: When not utilizing a model, such as in SVG(0) \citep{heess2015learning,amos2021model} and DDPG \citep{lillicrap2015continuous}, states are sampled from $\nu_\pi$; while when unrolling the model over full sequences, as in BPTT, states are sampled from the initial distribution.
%Then we have the following bound of gradient bias.
%Assumption \ref{reg_assumption} is mild when the truncation step is properly selected. 
% and redefine $\mathbb{P}(s_i, a_i)$, $\mathbb{P}(\hat{s}_i, \hat{a}_i)$ in \eqref{error_model_def}, \eqref{error_critic_def} with $s_0\sim\nu$. Then we are able to remove Assumption \ref{reg_assumption} and obtain the same gradient bias bound as in \eqref{eq::b_t_bound_DP} except without $\kappa'$.

Given that the effects of policy actions extend to all future states and rewards, unless we know the exact policy value function, its gradient $\nabla_\theta Q^{\pi_\theta}$ cannot be simply represented by quantities in any finite timescale. Hence, differentiating through a single critic function requires extra attention, as the true value gradient has recursive structures. To tackle this issue, we provide the gradient bias bound below that is based on the measure of discrepancy between the initial distribution $\zeta$ and the state visitation $\nu_\pi$.

\begin{proposition}[Gradient Bias]
\label{prop_grad_bias}
%Under Assumption TODO, for any $t\in[T]$, the gradient bias for \eqref{DP_ge} is bounded by
%$\kappa := \sup_{t\in[1, T]}\EE_{\nu_{\pi_t}}[(\ud\zeta / \ud\nu_{\pi_t}(s))^2]^{1/2}$
We denote $\kappa = \sup_{\pi}\EE_{\nu_{\pi}}[(\ud\zeta / \ud\nu_{\pi}(s))^2]^{1/2}$, where $\ud\zeta / \ud\nu_{\pi}$ is the Radon-Nikodym derivative of $\zeta$ with respect to $\nu_{\pi}$. Let $\kappa' = \beta + \kappa\cdot(1 - \beta)$. Under Assumption \ref{lip_assumption}, for any $t\in[T]$, the gradient bias is bounded by
\$
b_t = O\Bigl(\kappa\kappa'h^2(1 - \gamma^h) \Tilde{L}_{\hat{f}}^{h} \Tilde{L}_{f}^{h} \Tilde{L}_\pi^{2h}\epsilon_{f,t} / (1 - \gamma) + \kappa' h\gamma^{3h}\Tilde{L}_{\hat{f}}^{h}\Tilde{L}_\pi^h\epsilon_{v,t} / (1 -\gamma)^2\Bigr),
%O\Bigl(h^4 L_{\hat{f}}^{3h}L_\pi^h(\epsilon_f + \Tilde{L}_\pi^h) + \kappa' h^2\gamma^h L_{\hat{f}}^{2h}L_\pi^h\epsilon_v\Bigr).
%L_\pi \Biggl(2 L + O\Bigl(\epsilon_f\cdot r_{\text{max}}\cdot\frac{\gamma\cdot(1 - \gamma^h)}{1 - \gamma} + (1 - \gamma)\cdot\gamma^h\cdot (L_{\hat{Q}}\cdot h\cdot\epsilon_f + \epsilon_Q)\Bigr)\Biggr).
\$
where $\epsilon_{f,t}$ and $\epsilon_{v,t}$ are the shorthand notations of $\epsilon_{f}(t)$ defined in \eqref{error_model_def} and $\epsilon_v(t)$ in \eqref{error_critic_def}, respectively.
\end{proposition}
\vspace{-0.1cm}
The analysis above yields the identification of an optimal model expansion step $h^*$ that achieves the best convergence rate, whose form is presented by the following proposition.
%\yan{Suppose  true model $f$ is highly nonsmooth in a set with small measure ($L_f \gg 1$), it looks like we can do planning with a smooth approximation $\hat{f}$, where $L_{\hat{f}} \ll L_f$, so that planning with this approximation $\hat{f}$ has much smaller variance than planning under $f$, while only marginally increasing bias \eqref{eq::b_t_bound_DP}?}
%Even millions of samples would not suffice to give reliable gradient estimations and fail in simple tasks \citep{parmas2018pipps}.
%(One potential way to mitigate it is to constrain the Jacobian of the learned dynamical system \citep{metz2021gradients}. In other words, we can learn a more well-behaved non-chaotic version of physics instead of the rigid body dynamics with sharp changes.)


%[Clearly, if $L_{\hat{f}}>1$ and $L_f>1$, both the gradient bias and the gradient variance will increase exponentially, resulting in the optimal model expansion step $h^* = 0$, corresponding to not using the learned model at all. For this reason, it is common to assume $L_f<1$ in real systems for stable control. Therefore, the trade-off between gradient bias and variance results in a reasonable $h^*\in(0,\infty)$. TODO]

\begin{proposition}[Optimal Model Expansion Step]
\label{prop::optimal_h}
Given $L_f\leq 1$, if we regularize the model and policy so that $L_{\hat{f}}\leq 1$ and $L_\pi\leq 1$, then when $\gamma\approx 1$, the optimal model expansion step $h^*$ at iteration $t$ that minimizes the convergence rate upper bound satisfies $h^* = \max\{h'^*, 0\}$, where $h'^* = O(\epsilon_{v,t} / ((1-\gamma)(\epsilon_{f,t} + \epsilon_{v,t})))$ scales linearly with $\epsilon_{v,t} / (\epsilon_{f,t} + \epsilon_{v,t})$ and the effective task horizon $1 / (1-\gamma)$.
\end{proposition}
\vspace{-0.1cm}
In Proposition \ref{prop::optimal_h}, the Lipschitz condition of the underlying dynamics, i.e., $L_f\leq 1$, ensures the stability of the system. This can be seen in the linear system example, where the transitions are determined by the eigenspectrum of the family of transformations, leading to exponential divergence of trajectories w.r.t. the largest eigenvalue. In cases where this condition is not met in practical control systems, finding the best model unroll length may require trial and error. Fortunately, we have observed through experimentation that enforcing smoothness offers a much wider range of unrolling lengths that still provide satisfactory results.

\begin{remark}
As the error scale $\epsilon_{v,t} / (\epsilon_{f,t} + \epsilon_{v,t})$ increases, so too does the value of $h^*$. This finding can inform the practical algorithms to rely more on the model by performing longer unrolls when the model error $\epsilon_{f, t}$ is small, while avoiding long unrolls when the critic error $\epsilon_{v,t}$ is small.
\end{remark}
\vspace{-0.2cm}
Finally, we characterize the algorithm convergence rate.
\begin{corollary}[Convergence Rate]
\label{coro_con}
Let $\varepsilon(T) = \sum_{t=0}^{T-1}b_t$. We have for $T \geq 4L^2$ that
\$
\min_{t\in[T]}\EE\Bigl[\big\|\nabla_{\theta}J(\pi_{\theta_t})\big\|_2^2\Bigr] \leq 16\delta\cdot\varepsilon(T) / \sqrt{T}+ 4\varepsilon^2(T) / T + O\bigl(1 / \sqrt{T}\bigr).
\$
\end{corollary}
\vspace{-0.2cm}
The convergence rate can be further clarified by determining how quickly the errors of model and critic approach zero, i.e., $\sum_{t=0}^{T-1}\epsilon_f(t) + \epsilon_v(t)$. Such results can be accomplished by conducting a more fine-grained investigation of the model and critic function classes, such as utilizing overparameterized neural nets with width scaling with $T$ to bound the training error, as done in \cite{cai2019neural,liu2019neural}, and incorporating complexity measures of the model and critic function classes to bound $\epsilon_f(t)$ and $\epsilon_v(t)$. Their forms, however, are beyond the scope of this paper.

%\vskip1pt
\noindent{\bf A Spectral Normalization Method.} To ensure a smooth transition and faster convergence, we propose using a Spectral Normalization (SN) \citep{miyato2018spectral} model-based RP PGM that applies SN to all layers of the deep model network and policy network. While other techniques, such as adversarial regularization \citep{shen2020deep}, exist, we focus primarily on SN as it directly regulates the Lipschitz constant of the function. Specifically, the Lipschitz constant $L_g$ of a function $g$ satisfies $L_g = \sup_x \sigma_{\text{max}}(\nabla g(x))$, where $\sigma_{\text{max}}(W)$ denotes the largest singular value of the matrix $W$, defined as $\sigma_{\text{max}}(W) = \max_{\|x\|_2\leq 1}\|Wx\|_2$. For neural network $f$ with linear layers $g(x) = W_i x$ and $1$-Lipschitz activation (e.g., ReLU and leaky ReLU), we have $L_g = \sigma_{\text{max}}(W_i)$ and $L_{\hat{f}}\leq \prod_i\sigma_{\text{max}}(W_i)$. By normalizing the spectral norm of $W_i$ with $W^{\text{SN}}_i = W_i / \sigma_{\text{max}}(W_i)$, SN guarantees that the Lipschitz of $f$ is upper-bounded by $1$.



\iffalse
\begin{proposition}[Global Optimality of Stationary Point]
\label{prop::opt_stat_pt}
The stationary point $\hat{\theta}$ satisfies
\#
(1 - \gamma)\cdot\bigl(J(\pi^*) - J(\pi_{\hat{\theta}})\bigr) \leq 2r_{\text{max}}\cdot \inf_{\theta}\Big\|u_{\hat{\theta}}(s, a) - \bigl(\nabla_\theta\log\pi_{\hat{\theta}}(a|s)\bigr)^\top \theta\Big\|_{\sigma_{\pi_{\hat{\theta}}}},
\#
where $u_{\hat{\theta}}: \mathcal{S}\times\mathcal{A}\rightarrow \mathbb{R}$ is defined as
\$
u_{\hat{\theta}}(s, a) := \frac{d\sigma_{\pi^*}}{d\sigma_{\pi_{\hat{\theta}}}}(s, a) - \frac{d\nu_{\pi^*}}{d\nu_{\pi_{\hat{\theta}}}}(s), \,\,\forall (s, a)\in\mathcal{S}\times\mathcal{A}.
\$
Here, $d\sigma_{\pi^*} / d\sigma_{\pi_{\hat{\theta}}}$ and $d\nu_{\pi^*} / d\nu_{\pi_{\hat{\theta}}}$ are the Radon-Nikodym derivatives and $\|\cdot\|_{\sigma_{\pi_{\hat{\theta}}}}$ is the $L_2(\sigma_{\pi_{\hat{\theta}}})$-norm.
\end{proposition}
TODO
\fi

%While the above analysis gives a unified convergence rate of the two gradient estimators in \eqref{DP_ge} and \eqref{DR_ge}, we provide a more fine-grained investigation below.

%\begin{corollary}[Comparison between the two gradient estimators]
%Gradient Lipschitz assumption TODO.
%\end{corollary}


%\subsection{Existing Problems}
%\begin{itemize}
%    \item Convergence rate requires sublinear $\sum_{t=1}^T b_t^2 + v_t$.
%    \item Under what conditions does Prop. \ref{prop::opt_stat_pt} indicate global optimality.
%    \item Optional: How \eqref{error_model_def} relates to conventional definition of model error.
%\end{itemize}
